Characterizing the Effects of Translation on Intertextuality using Multilingual Embedding Spaces

Rhetorical devices are difficult to translate, but they are crucial to the translation of literary documents. We investigate the use of multilingual embedding spaces to characterize the preservation of intertextuality, one common rhetorical device, across human and machine translation. To do so, we use Biblical texts, which are both full of intertextual references and are highly translated works. We provide a metric to characterize intertextuality at the corpus level and provide a quantitative analysis of the preservation of this rhetorical device across extant human translations and machine-generated counterparts. We go on to provide qualitative analysis of cases wherein human translations over- or underemphasize the intertextuality present in the text, whereas machine translations provide a neutral baseline. This provides support for established scholarship proposing that human translators have a propensity to amplify certain literary characteristics of the original manuscripts.

==> New_Tables/it_ratios.tex <==
\section{Intertextuality ratios}
\label{appendix:intertextuality}
\begin{table*}[h]
\centering
\small
\begin{tabular}{lllr}
\toprule
%   &  &  \multicolumn{2}{c}{Ratio} \\
Condition & Manuscript & Language & Ratio \\
\midrule
%\multirow[t]{56}{*}{Jewish} 
\multirow[c]{2}{*}{original} & WLC & Hebrew & 1.430 \\
%\cline{2-3} \cline{3-4}
 & Sinaiticus & Greek & 1.169 \\
\cline{1-4} %\cline{2-3} \cline{3-4}
\multirow[c]{5}{*}{human translation} & \multirow[c]{5}{*}{BC} & English & 1.587 \\
%\cline{4-4}
&  & Finnish & 1.458 \\
%\cline{4-4}
&  & Marathi & 1.371 \\
%\cline{3-4}
&  & Swedish & 1.360 \\
%\cline{3-4}
&  & Turkish & 1.449 \\
\cline{1-4}
%\cline{3-4} %\cline{3-6} \cline{4-6}
\multirow[c]{10}{*}{unconstrained} & \multirow[c]{5}{*}{WLC} & English & 1.536 \\
%\cline{4-6}
  &  & Finnish & 1.327 \\
%\cline{4-6}
  &  & Marathi & 1.340 \\
%\cline{4-6}
  &  & Swedish & 1.244 \\
%\cline{4-6}
  &  & Turkish & 1.278 \\
%\cline{3-6} \cline{4-6}
\cline{2-4}
  & \multirow[c]{5}{*}{Sinaiticus} & English & 1.342 \\
%\cline{4-6}
  &  & Finnish & 1.234 \\
%\cline{4-6}
  &  & Marathi & 1.240 \\
%\cline{4-6}
  &  & Swedish & 1.176 \\
%\cline{4-6}
  &  & Turkish & 1.208 \\
%\cline{2-6} \cline{3-6} \cline{4-6}
\cline{1-4}
 \multirow[c]{10}{*}{exclude human} & \multirow[c]{5}{*}{WLC} & English & 1.456 \\
%\cline{4-6}
  &  & Finnish & 1.314 \\
%\cline{4-6}
  &  & Marathi & 1.267 \\
%\cline{4-6}
  &  & Swedish & 1.230 \\
%\cline{4-6}
  &  & Turkish & 1.288 \\
  \cline{2-4}
%\cline{3-6} \cline{4-6}
  & \multirow[c]{5}{*}{Sinaiticus} & English & 1.272 \\
%\cline{4-6}
  &  & Finnish & 1.186 \\
%\cline{4-6}
  &  & Marathi & 1.206 \\
%\cline{4-6}
  &  & Swedish & 1.138 \\
%\cline{4-6}
  &  & Turkish & 1.194 \\
  \cline{1-4}
%\cline{2-6} \cline{3-6} \cline{4-6}
 \multirow[c]{10}{*}{exclude references} & \multirow[c]{5}{*}{WLC} & English & 1.516 \\
%\cline{4-6}
  &  & Finnish & 1.326 \\
%\cline{4-6}
  &  & Marathi & 1.297 \\
%\cline{4-6}
  &  & Swedish & 1.224 \\
%\cline{4-6}
  &  & Turkish & 1.274 \\
%\cline{3-6} \cline{4-6}
\cline{2-4}
 & \multirow[c]{5}{*}{Sinaiticus} & English & 1.345 \\
%\cline{4-6}
&  & Finnish & 1.234 \\
%\cline{4-6}
 &  & Marathi & 1.190 \\
%\cline{4-6}
 &  & Swedish & 1.150 \\
%\cline{4-6}
  &  & Turkish &  1.193 \\
%\cline{2-6} \cline{3-6} \cline{4-6}
\cline{1-4}
 \multirow[c]{10}{*}{exclude both} & \multirow[c]{5}{*}{WLC} & English & 1.448 \\
%\cline{4-6}
  &  & Finnish & 1.317 \\
%\cline{4-6}
  &  & Marathi & 1.255 \\
%\cline{4-6}
  &  & Swedish & 1.206 \\
%\cline{4-6}
  &  & Turkish & 1.268 \\
%\cline{3-6} \cline{4-6}
\cline{2-4}
  & \multirow[c]{5}{*}{Sinaiticus} & English & 1.278 \\
%\cline{4-6}
  &  & Finnish & 1.185 \\
%\cline{4-6}
  &  & Marathi & 1.207 \\
%\cline{4-6}
  &  & Swedish & 1.140 \\
%\cline{4-6}
  &  & Turkish & 1.201 \\
  \bottomrule
%\cline{1-6} \cline{2-6} \cline{3-6} \cline{4-6}
\end{tabular}
\caption{Intertextuality ratios for editions and translations of the Jewish testament.}
\label{table:jewish}
\end{table*}

\begin{table*}
\centering
\small
\begin{tabular}{lllr}
\toprule
% &  &  &  &  \multicolumn{2}{c}{Ratio} \\
Condition & Manuscript & Language & Ratio \\
\midrule
original & Sinaiticus & Greek & 1.394 \\
\cline{1-4} % \cline{3-6} \cline{4-6}
\multirow[c]{5}{*}{human translation} & \multirow[c]{5}{*}{BC} & English & 1.666 \\
%\cline{2-4}
&  & Finnish & 1.438 \\
%\cline{4-6}
 &  & Marathi & 1.406 \\
%\cline{4-6}
  &  & Swedish & 1.373 \\
%\cline{4-6}
  &  & Turkish & 1.428 \\
  \cline{1-4}
%\cline{2-6} \cline{3-6} \cline{4-6}
\multirow[c]{5}{*}{unconstrained} & \multirow[c]{5}{*}{Sinaiticus} & English & 1.752 \\
%\cline{4-6}
  &  & Finnish & 1.351 \\
%\cline{4-6}
  &  & Marathi & 1.339 \\
%\cline{4-6}
  &  & Swedish & 1.298 \\
%\cline{4-6}
  &  & Turkish & 1.311 \\
\cline{1-4} %\cline{3-6} \cline{4-6}
\multirow[c]{5}{*}{exclude human} & \multirow[c]{5}{*}{Sinaiticus} & English & 1.624 \\
%\cline{4-6}
 &  & Finnish & 1.348 \\
%\cline{4-6}
&  & Marathi & 1.316 \\
%\cline{4-6}
 &  & Swedish & 1.271 \\
%\cline{4-6}
 &  & Turkish & 1.281 \\
\cline{1-4} %\cline{3-6} \cline{4-6}
\multirow[c]{5}{*}{exclude references} & \multirow[c]{5}{*}{Sinaiticus} & English & 1.646 \\
%\cline{4-6}
  &  & Finnish & 1.347 \\
%\cline{4-6}
  &  & Marathi & 1.305 \\
%\cline{4-6}
  &  & Swedish & 1.255 \\
%\cline{4-6}
  &  & Turkish & 1.307 \\
\cline{1-4} %\cline{3-6} \cline{4-6}
\multirow[c]{5}{*}{exclude both} & \multirow[c]{5}{*}{Sinaiticus} & English & 1.639 \\
%\cline{4-6}
  &  & Finnish & 1.353 \\
%\cline{4-6}
  &  & Marathi & 1.299 \\
%\cline{4-6}
  &  & Swedish & 1.261 \\
%\cline{4-6}
  &  & Turkish & 1.293 \\
  \bottomrule
%\cline{1-6} \cline{2-6} \cline{3-6} \cline{4-6}
\end{tabular}
\caption{Intertextuality ratios for editions and translations of the Christian testament.}
\label{table:christian}
\end{table*}

\begin{table*}
\centering
\small
\begin{tabular}{llllr}
\toprule
% &  &  &  &  \multicolumn{2}{c}{Ratio} \\
Condition & Manuscript & Language & Type & Ratio \\
\midrule
\multirow[c]{2}{*}{original} & \multirow[c]{2}{*}{Sinaiticus} & \multirow[c]{3}{*}{Greek} & endo & 1.306 \\
  &  &  & exo & 1.313 \\

%\cline{2-6} \cline{3-6} \cline{4-6}
\cline{1-5}
 
 \multirow[c]{10}{*}{human translation} & \multirow[c]{10}{*}{BC} & \multirow[c]{2}{*}{English} & endo & 1.635 \\
  &  &  & exo & 1.728 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Finnish} & endo & 1.445 \\
  &  &  & exo & 1.469 \\
\cline{4-5}
 &  & \multirow[c]{2}{*}{Marathi} & endo & 1.393 \\
 &  &  & exo & 1.433 \\
\cline{4-5}
&  & \multirow[c]{2}{*}{Swedish} & endo & 1.368 \\
&  &  & exo & 1.370 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Turkish} & endo & 1.435 \\
  &  &  & exo & 1.490 \\
\cline{1-5}
 \multirow[c]{10}{*}{unconstrained} & \multirow[c]{10}{*}{Sinaiticus} & \multirow[c]{2}{*}{English} & endo & 1.582 \\
  &  &  & exo & 1.642 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Finnish} & endo & 1.308 \\
  &  &  & exo & 1.272 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Marathi} & endo & 1.304 \\
  &  &  & exo & 1.305 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Swedish} & endo & 1.254 \\
  &  &  & exo & 1.217 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Turkish} & endo & 1.274 \\
  &  &  & exo & 1.286 \\
\cline{1-5}
 \multirow[c]{10}{*}{exclude human} & \multirow[c]{10}{*}{Sinaiticus} & \multirow[c]{2}{*}{English} & endo & 1.474 \\
 &  &  & exo & 1.550 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Finnish} & endo & 1.288 \\
  &  &  & exo & 1.270 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Marathi} & endo & 1.276 \\
  &  &  & exo & 1.259 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Swedish} & endo & 1.222 \\
  &  &  & exo & 1.195 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Turkish} & endo & 1.251 \\
  &  &  & exo & 1.293 \\
\cline{1-5}
 \multirow[c]{10}{*}{exclude references} & \multirow[c]{10}{*}{Sinaiticus} & \multirow[c]{2}{*}{English} & endo & 1.521 \\
  &  &  & exo & 1.616 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Finnish} & endo & 1.305 \\
  &  &  & exo & 1.288 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Marathi} & endo & 1.263 \\
  &  &  & exo & 1.250 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Swedish} & endo & 1.217 \\
  &  &  & exo & 1.192 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Turkish} & endo & 1.265 \\
  &  &  & exo & 1.263 \\
\cline{1-5}
 \multirow[c]{10}{*}{exclude both} & \multirow[c]{10}{*}{Sinaiticus} & \multirow[c]{2}{*}{English} & endo & 1.485 \\
  &  &  & exo & 1.583 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Finnish} & endo & 1.291 \\
  &  &  & exo & 1.286 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Marathi} & endo & 1.265 \\
  &  &  & exo & 1.252 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Swedish} & endo & 1.216 \\
  &  &  & exo & 1.194 \\
\cline{4-5}
  &  & \multirow[c]{2}{*}{Turkish} & endo & 1.260 \\
  &  &  & exo & 1.273 \\
\bottomrule
\end{tabular}
\caption{Intertextuality ratios for editions and translations of both testaments.}
\label{table:both}
\end{table*}

==> New_Tables/summary.tex <==
\begin{table}
\caption{Inter-textuality scores of human translations}
\begin{tabular}{lr}
\toprule
Language & Score \\
\midrule
English & 1.23 \\
French & 1.22 \\
Swedish & 1.25 \\
Turkish & 1.27 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from source language human translation with masked vocabulary from both human and referent translations}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.07 & -0.08 & -0.20 &  \\
French &  & 0.71 & 0.05 & -0.07 \\
Swedish & 0.32 &  & 0.56 & 0.02 \\
Turkish & -0.03 & 0.70 &  & 0.11 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from target language human translation with masked vocabulary from both human and referent translations}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.03 & 0.02 & 0.01 &  \\
French &  & 0.75 & 0.24 & -0.03 \\
Swedish & 0.22 &  & 0.60 & -0.08 \\
Turkish & -0.31 & 0.67 &  & -0.08 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from source language human translation with masked vocabulary from human translation}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.01 & -0.25 & -0.23 &  \\
French &  & 0.05 & -0.34 & -0.16 \\
Swedish & 0.39 &  & 0.22 & 0.04 \\
Turkish & 0.40 & 0.34 &  & 0.07 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from target language human translation with masked vocabulary from human translation}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & -0.03 & -0.14 & -0.01 &  \\
French &  & 0.17 & -0.06 & -0.11 \\
Swedish & 0.31 &  & 0.29 & -0.06 \\
Turkish & 0.25 & 0.27 &  & -0.13 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from source language human translation with no vocabulary masking}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.05 & -0.29 & -0.22 &  \\
French &  & -0.01 & 0.06 & -0.10 \\
Swedish & 0.10 &  & 0.30 & 0.13 \\
Turkish & 0.81 & 0.46 &  & -0.00 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from target language human translation with no vocabulary masking}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.01 & -0.17 & -0.00 &  \\
French &  & 0.11 & 0.25 & -0.06 \\
Swedish & -0.02 &  & 0.36 & 0.04 \\
Turkish & 0.76 & 0.40 &  & -0.22 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from source language human translation with masked vocabulary from translations of referent sentences}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.04 & -0.34 & -0.21 &  \\
French &  & 0.58 & 0.24 & -0.14 \\
Swedish & 0.17 &  & 0.39 & 0.01 \\
Turkish & 0.20 & 0.65 &  & 0.12 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Percent-delta from target language human translation with masked vocabulary from translations of referent sentences}
\begin{tabular}{lrrrr}
\toprule
Source & French & Swedish & Turkish & English \\
\midrule
English & 0.01 & -0.22 & 0.00 &  \\
French &  & 0.63 & 0.40 & -0.10 \\
Swedish & 0.05 &  & 0.45 & -0.08 \\
Turkish & -0.01 & 0.62 &  & -0.07 \\
\bottomrule
\end{tabular}
\end{table}


